Private Data Valuation and Fair Payment in Data Marketplaces

Data valuation is an essential task in a data marketplace. It aims at fairly compensating data owners for their contribution. There is increasing recognition in the machine learning community that the Shapley value -- a foundational profit-sharing scheme in cooperative game theory -- has major potential to value data, because it uniquely satisfies basic properties for fair credit allocation and has been shown to be able to identify data sources that are useful or harmful to model performance. However, calculating the Shapley value requires accessing original data sources. It still remains an open question how to design a real-world data marketplace that takes advantage of the Shapley value-based data pricing while protecting privacy and allowing fair payments. In this paper, we propose the {\em first} prototype of a data marketplace that values data sources based on the Shapley value in a privacy-preserving manner and at the same time ensures fair payments. Our approach is enabled by a suite of innovations on both algorithm and system design. We firstly propose a Shapley value calculation algorithm that can be efficiently implemented via multiparty computation (MPC) circuits. The key idea is to learn a performance predictor that can directly predict model performance corresponding to an input dataset without performing actual training. We further optimize the MPC circuit design based on the structure of the performance predictor. We further incorporate fair payment into the MPC circuit to guarantee that the data that the buyer pays for is exactly the same as the one that has been valuated. Our experimental results show that the proposed new data valuation algorithm is as effective as the original expensive one. Furthermore, the customized MPC protocol is efficient and scalable.

==> sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\paragraph{Extending to evaluate labeled dataset}
The labeled pre-sharing method and the unlabeled pre-sharing method are mainly suitable for evaluating the utility of unlabeled datasets. In fact, the labeled pre-sharing method can be easily extended to evaluate labeled datasets. The core idea is to incorporate the knowledge of labels into training the utility function. A straight method is to put the output of the feature extractor $G_f$ and one-hot vector of the label together, and input them to the DeepSets model $F_{DS}$. With the help of label knowledge, the utility function could have better performance on evaluation the utility of datasets. We experiment with the CIFAR-10 dataset. The results is shown in Figure~\ref{fig:discussion_label}.

\begin{figure}
\centering
\setlength\tabcolsep{1.0pt}
    \subfloat[Removing low value data]{
        \includegraphics[width=0.24\textwidth,valign=c]{./plot/cifar10_label_l2h.png}}
    \subfloat[Removing high value data]{
        \includegraphics[width=0.24\textwidth,valign=c]{./plot/cifar10_label_h2l.png}} 
\caption{Comparison of evaluating labeled datasets and unlabeled datasets }
\label{fig:discussion_label}
\end{figure}

